Onboard View Planning of a Flying Camera for High Fidelity 3D Reconstruction of a Moving Actor

Capturing and reconstructing a human actor's motion is important for filmmaking and gaming. Currently, motion capture systems with static cameras are used for pixel-level high-fidelity reconstructions. Such setups are costly, require installation and calibration and, more importantly, confine the user to a predetermined area. In this work, we present a drone-based motion capture system that can alleviate these limitations. We present a complete system implementation and study view planning which is critical for achieving high-quality reconstructions. The main challenge for view planning for a drone-based capture system is that it needs to be performed during motion capture. To address this challenge, we introduce simple geometric primitives and show that they can be used for view planning. Specifically, we introduce Pixel-Per-Area (PPA) as a reconstruction quality proxy and plan views by maximizing the PPA of the faces of a simple geometric shape representing the actor. Through experiments in simulation, we show that PPA is highly correlated with reconstruction quality. We also conduct real-world experiments showing that our system can produce dynamic 3D reconstructions of good quality. We share our code for the simulation experiments in the link: https://github.com/Qingyuan-Jiang/view_planning_3dhuman

==> sections/motivating_scenario.tex <==
% This section will describe a motivating scenario for our drone system. As shown in Fig. \ref{fig:concept_figure}, there is one dynamic moving person as the reconstruction object in this scenario. We have one flying drone recording video with an onboard RGB-D camera during the flight. During offline post-processing, we use the camera readings to obtain a high-fidelity model of humans, such as point clouds or mesh.

% To simplify the problem, we assume the actor's movement is constrained, such that the actor is kept in the camera's field of view (FOV). \vtxt{how is this assumption justified?}

% Because the actor is dynamic, such as walking and dancing, only limited consecutive views are available. We need to place each view in a good position and orientation. The actor's pose is therefore required to plan the views. 

% In Sec.~\ref{sec:formulation}, we start with planning views for high-fidelity reconstruction and formulate the problem with the actor and drone's pose representation. We solve the problem in Sec.~\ref{sec:system}, where we also introduce the entire system by each module. In Sec.~\ref{sec:experiments} we conduct experiments to examine each module separately and show our reconstruction of dynamic actor results.

% \vtxt{this section is confusing to me. Are you trying to explain the challenges?}https://www.overleaf.com/project/630b8de1d07fa7f640a43a4e
